Microsecond-scale Dynamic Validation of Idempotency for GPU Kernels

We discovered that a GPU kernel can have both idempotent and non-idempotent instances depending on the input. These kernels, called conditionally-idempotent, are prevalent in real-world GPU applications (490 out of 547 from six applications). Consequently, prior work that classifies GPU kernels as either idempotent or non-idempotent can severely compromise the correctness or efficiency of idempotence-based systems. This paper presents PICKER, the first system for instance-level idempotency validation. PICKER dynamically validates the idempotency of GPU kernel instances before their execution, by utilizing their launch arguments. Several optimizations are proposed to significantly reduce validation latency to microsecond-scale. Evaluations using representative GPU applications (547 kernels and 18,217 instances in total) show that PICKER can identify idempotent instances with no false positives and a false-negative rate of 18.54%, and can complete the validation within 5 us for all instances. Furthermore, by integrating PICKER, a fault-tolerant system can reduce the checkpoint cost to less than 4% and a scheduling system can reduce the preemption latency by 84.2%.

==> impl.tex <==
\section{Implementation}

We have implemented {\sys} with 10k lines of Python for the static analyzer
and 1k lines of C++ for the runtime validator.
The analyzer in {\sys} was implemented to analyze assembly code of GPU kernels,
which first works on ISA of NVIDIA Volta GPUs (e.g., GV100 in our experiments).
Choosing to support assembly language instead of source code enables {\sys} to analyze 
close-sourced GPU kernels (e.g., GPU kernels from cuDNN~\cite{Chetlur2014cuDNNEP}).
The symbolic execution engine is implemented based on claripy~\cite{Shoshi2016SoK} and
Z3~\cite{Moura2008Z3AE}.

Besides the optimization techniques that aims to achieve the {\us}-scale validation latency
discussed in $\S$\ref{sec:opt}, we also implemented a few other techniques to
speed up the static analysis. For example, before symbolic execution, {\sys} first
performs a data flow analysis to identify the instructions that are not related to
the memory access instructions~\cite{Li2014PracticalSR}, and then skip them during symbolic execution.


==> rev.tex <==
\gdef\therev{de9cd82}
\gdef\thedate{2024-10-31 13:40:09 +0800}

